Center-Embedding and Constituency in the Brain and a New Characterization of Context-Free Languages

A computational system implemented exclusively through the spiking of neurons was recently shown capable of syntax, that is, of carrying out the dependency parsing of simple English sentences. We address two of the most important questions left open by that work: constituency (the identification of key parts of the sentence such as the verb phrase) and the processing of dependent sentences, especially center-embedded ones. We show that these two aspects of language can also be implemented by neurons and synapses in a way that is compatible with what is known, or widely believed, about the structure and function of the language organ. Surprisingly, the way we implement center embedding points to a new characterization of context-free languages.

==> pseudocode.tex <==


\begin{algorithm}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{a sentence $s$}
\Output{representation of dependency parse of $s$, rooted in {\sc Verb}}
\BlankLine
 disinhibit({\sc Lex}, 0) \;
 disinhibit({\sc Subj}, 0) \;
 disinhibit({\sc Verb}, 0) \;
 \ForEach{\upshape word $w$ in $s$}{
  activate assembly $x_w$ in {\sc Lex} \;
  \ForEach{\upshape pre-rule (Dis)inhibit($\square,i$) in $\alpha_w \rightarrow$ Pre-Commands}{
    (Dis)inhibit($\square, i$) \;
  }
  }
 {\em project}* \;  
 \ForEach{\upshape post-rule (Dis)inhibit($\square,i$) in $\alpha_w \rightarrow$ Post-Commands}{
    (Dis)inhibit($\square, i$)
  }
\BlankLine
 \caption{Parser, main loop}
\end{algorithm}

\begin{algorithm}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
\Input{$G$ after parsing, with active root assembly $v$ in {\sc Verb}}
\Output{the parse tree stored implicitly in $G$}
\BlankLine
initialize stack $s$ as \{$(v,{\textsc Verb})$\} \;
initialize dependencies $\mathcal{D} = \{\}$ \;
 \While{\upshape $s$ not empty }{
  ($x$,$A$) = $s$.pop() \;
  {\em project}($x$, {\sc Lex}) \;
  $w_A$ = {\em getWord}() \;
  \ForEach{\upshape area $B \neq A$ s.t. $(A,B) \in \mathcal{F}$}{
  $y$ = {\em try-project}$(x,B)$ \;
  \If{$y$ not None}{
  {\em project}($y$, {\sc Lex}) \;
  $w_B$ = {\em getWord}() \;
  add dependency $w_A \xrightarrow{B} w_B$ to $\mathcal{D}$ \;
  s.insert($(y,B)$) \;
  }
  }
 }
 return $\mathcal{D}$ \;
 \caption{Read out of parse tree in $G$}
\end{algorithm}



\begin{algorithm}
\BlankLine
\ForEach{\upshape area $A$}{
    \If{\upshape there is active assembly $x$ in $A$}{
    \ForEach{$i \in x$}{
        $f_i^1 = 1$ \;
    }
    }
}
\BlankLine
\For{$i=1,\ldots,20$}{
all $A$, all $i\in A$, initialize $SI_i^t = 0$ \;
\ForEach{\upshape uninhibited areas $A$, $B$}{
    \If{\upshape fiber $(A,B)$ inhibited}{
		skip \;
	}
	$x = \{i \in A : f_i^t = 1\}$ \;
	\ForEach{\upshape $j \in B$}{
		$SI_j^t$ += $\sum_{i \in x, (i,j)\in E} w_{ij}$ \;
	}
}
\BlankLine
\ForEach{\upshape uninhibited area $A$}{
	\ForEach{\upshape $i \in A$}{
	\eIf{\upshape $SI_i^t$ in top$-k_{j\in A}(SI_j^t)$ }{
			$f_i^{t+1}$ = 1 \;
	}{
		$f_i^{t+1}$ = 0 \;
	}
	}
}
\ForEach{\upshape uninhibited areas $A$,$B$}{
    \If{\upshape fiber $(A,B)$ inhibited}{
		skip \;
	}
	\ForEach{\upshape $(i,j) \in (A\times B)\cap E$}{
    \If{\upshape $f_i^t = 1$ and $f_j^{t+1}=1$}{
        $w_{ij}$ = $w_{ij} \times (1+\beta)$
    }
	}
}
}
\caption{AC code for project*}
\end{algorithm}


\begin{figure*} 
  \includegraphics[scale=0.9, trim=50 70 0 0, clip]{parser_figure3.pdf}
  \caption{Trace of the Parser for the sentence {\em ``the man saw a woman"}. The action $\alpha_i$ of each word is given beneath a figure showing the state of the Parser after the Pre-commands and project* have occurred for that word. Green areas and fiber arrows are disinhibited; red are inhibited. All assemblies active right after project* are shown (with the one in {\sc Lex} labeled $x_w$). Purple dotted arrows indicate assemblies that have been connected; one can fire to activate the other. Purple arrows to {\sc Lex} are shown only in the stage in which they are created. Green ($\color{green}{\bm{\ocircle}}$) and red ($\color{red}\bm{\oslash}$) circles indicate areas or fibers that will be disinhibited/inhibited by the Post-commands.}
  \label{fig:big}
\end{figure*}

@article{neuro,
title = {Interactions between attention and working memory},
journal = {Neuroscience},
volume = {139},
number = {1},
pages = {201-208},
year = {2006},
issn = {0306-4522},
doi = {https://doi.org/10.1016/j.neuroscience.2005.08.023},
url = {https://www.sciencedirect.com/science/article/pii/S0306452205008985},
author = {E. Awh and E.K. Vogel and S.-H. Oh},
keywords = {attention, working memory},
}
